A Balanced Approach of Rapid Genetic Exploration and Surrogate Exploitation for Hyperparameter Optimization

This paper proposes a new method for hyperparameter optimization (HPO) that balances exploration and exploitation. While evolutionary algorithms (EAs) show promise in HPO, they often struggle with effective exploitation. To address this, we integrate a linear surrogate model into a genetic algorithm (GA), allowing for smooth integration of multiple strategies. This combination improves exploitation performance, achieving an average improvement of 1.89 percent (max 6.55 percent, min -3.45 percent) over existing HPO methods.

==> algorithms/fga.tex <==
\begin{algorithm}[htbp]
\caption{Rapid Genetic Exploration}
\begin{algorithmic}[1]
    \renewcommand{\algorithmicrequire}{\textbf{parameter(s):}}
    \renewcommand{\algorithmicensure}{\textbf{output:}}
    \REQUIRE $F$ - Fitness function, $\alpha$ - Intensity factor of probability
    \ENSURE  Best individual
\\ \textit{Initialisation}
    \STATE $D$←Empty list 
    \COMMENT {Experience memory}
    \STATE $P$←RANDOM-POPULATION($P$)
    \STATE Store transition ($P$ , $F(P)$) in $D$
\\ \textit{Loop process} 
    \REPEAT
        \STATE $P'$←Empty list
        \FOR {i = 1 to SIZE(P)}
            \STATE $p_1$, $p_2$←TOP-N-RANDOM-CHOICES(P, 2)
            \COMMENT {$p$: Parent}
            \STATE $o_1$←$p_1$, $o_2$←$p_2$
            \COMMENT {$o$: Offspring}
            \STATE $n$←LENGTH($p_1$)
            \STATE $m$←Random number from 1 to $n$
            \STATE $c$←RANDOM-CHOICES([1:$n$], $m$)
            \FOR { $i$ = 1 to $n$}
                \IF {$i$ in $c$}
                    \STATE $o_1[i]$←$o_2[i]$, $o_2[i]$←$o_1[i]$
                \ENDIF
            \ENDFOR
            \COMMENT {Multi-crossover}
            \STATE $\beta$←SLOPE($D$)
            \COMMENT {Slope of fitness scores}
            \STATE $\delta$← $1.5 - {1}/{(1 + e^{-\alpha\cdot|\beta|})} $
            \COMMENT {Equation (1)}
            \STATE $r$←RANDOM()
            \IF {$\delta \ge r$} 
                \STATE $o_1$, $o_2$←MULTI-MUTATE($o_1$, $o_2$)
            \ENDIF
            \STATE add $o_1$, $o_2$ to $P'$
            \STATE Store transition ($P'$ , $F(P')$) in $D$
        \ENDFOR
        \STATE $P$←$P'$
    \UNTIL{Some individual is ﬁt enough, or enough time has elapsed}
    \RETURN Best individual in $P$
\end{algorithmic} 
\end{algorithm}

==> algorithms/prim.tex <==
\begin{algorithm}[htbp]
\caption{Deep Pseudo-Reverse Identification MIMO(PRIM)}
\begin{algorithmic}[1]
    \renewcommand{\algorithmicrequire}{\textbf{parameter(s):}}
    \renewcommand{\algorithmicensure}{\textbf{output:}}
    \REQUIRE $P$ - Population, $R$ - Fitness scores, $C$ - Number of Estimated individuals
    \ENSURE  estimated individuals
\\ \textit{Initialisation}
    \STATE $X \gets R^{K}$, $y \gets P^{K}$
    \COMMENT  {Reverse}
    \STATE $T$←UNIFORM-NOISES(0:1, $K$)
    \STATE append $T$ to $X$, $y$
    \COMMENT  {Add Identification}
    \STATE $Q$←MIMO-Function with random weights $\theta$
    \STATE train $Q(X, y, \theta)$
    \STATE result←empty list
    \STATE $i^*$← arg max($y$)
    \STATE $x$← $Q([1, y[i^*][1]], \theta^*)$
    \STATE add $x[-1]$ to result
    \STATE delete $X[i^*], y[i^*]$
\\ \textit{Loop process}
    \REPEAT
        % \STATE $i^*$← arg max($y$)
        % \STATE $x$← $Q([1, y[i^*][1]], \theta^*)$
        \STATE $D$← empty list
        \FOR { i = 1 to SIZE(X)}
            \STATE $c$←PEARSON-CORRELATION($x[-1], X[i][-1]$)
            \STATE $x$←$Q([1, y[i][1]], \theta^*)$
            \STATE add ($c$, $x$) to $D$
        \ENDFOR
        \STATE $v$←median of $D.c$
        \REPEAT
            \STATE $i^*$← arg max($y$)
            \STATE delete $X[i^*], y[i^*], D[i^*]$
        \UNTIL {$D.c[i^*]$ $\le$ $v$}
        \STATE $x$← $Q([1, y[i][1]], \theta^*)$
        \STATE add $x[-1]$ to result
        
    \UNTIL {SIZE(result) = $C$, or enough time has elapsed}
    \RETURN the best individuals in MIMO-Function
   
\end{algorithmic} 
\end{algorithm}

==> algorithms/rghl.tex <==
\begin{algorithm}[htbp]
\caption{Rapid Genetic algorithm with random direction Hill-climbing Linear model(RGHL)}
\begin{algorithmic}[1]
    \renewcommand{\algorithmicrequire}{\textbf{parameter(s):}}
    \renewcommand{\algorithmicensure}{\textbf{output:}}
    \REQUIRE $F$ - Fitness function, $\psi$ - Number of Population, $\omega$ - Number of generations, $\xi$ - Number of best estimated individuals by RHCLM, $C$ - Num-
ber of Estimated individuals, $V$ - Number of steps
    \ENSURE  Best individual
\\ \textit{Initialisation}
    \STATE $D$← Empty list
    \COMMENT {Experience memory}
    \STATE $P$←RANDOM-POPULATION($\psi$ )
    \STATE Store transition ($P$, $F(P)$) in $D$
\\ \textit{Loop process} 
    \FOR { $i$ = 1 to $\omega$ }
        \STATE $P'$←Empty list
        \WHILE {SIZE($P'$) $\leq$ ($\psi$ - $\xi$)}
            \STATE $p_0$, $p_1$←TOP-N-RANDOM-CHOICES($P$)
            \STATE $o_0$, $o_1$←MULTI-CROSSOVER($p_0$, $p_1$)
            \STATE $o_0$, $o_1$←MULTI-MUTATE($o_0$, $o_1$)
            \COMMENT {With Equation (1)}
            \STATE add  $o_0$, $o_1$ to $P'$
        \ENDWHILE
        \COMMENT {Algorithm 1}
        \STATE $P$←$P'$, $R$←$F(P')$
        \STATE Store transition ($P$, $R$) in $D$
        \STATE $\pi$←RHCLM($D$, $C$, $V$)
        \COMMENT {Algorithm 2}
        \STATE add  $\pi$ to $P$
    \ENDFOR
    \RETURN Best individual in $P$
\end{algorithmic} 
\end{algorithm}

==> algorithms/rhc.tex <==
\begin{algorithm}[htbp]
    \caption{Random direction Hill-Climbing(RHC)}
    \begin{algorithmic}[1]
        \renewcommand{\algorithmicrequire}{\textbf{parameter(s):}}
        \renewcommand{\algorithmicensure}{\textbf{output:}}
        \REQUIRE $Q$ - Surrogate model, $C$ - Number of genes, $V$ - Number of steps, $U$ - Best individuals
        \ENSURE  $B$ - Estimated best individuals
    \\ \textit{Initialisation}
        \STATE $B \gets$ Empty list, $R \gets$ Empty list
        \COMMENT{$R$: Fitness scores}
    \\ \textit{Loop process}
        \FOR {$u$ in $U$}
            \FOR {$j$ = 1 to $V$}
                \STATE $r^{*} \gets 0$
                \COMMENT{Initialize optimal score}  
                \STATE $d \gets$ RANDOM-INT-ARRAY(-1, 1, $C$)
                \COMMENT{Generate random directions}
    
                \REPEAT
                    \STATE $h \gets u - d$
                    \COMMENT{Climbing}
                    \STATE $r \gets Q(h)$
                    \IF {$r^{*} >=  r$} 
                        \STATE add $h$ to $B$, add $r$ to $R$
                        \STATE $u \gets h$, $r^{*} \gets r$
                    \ENDIF
                \UNTIL{$h == u$}
            \ENDFOR
        \ENDFOR
        \STATE $B \gets$ SORT-BY-ASC-SCORE($B$, $R$)
        \STATE $B \gets B[1:SIZE(U)] $
        \RETURN $B$
       
    \end{algorithmic} 
\end{algorithm}





==> algorithms/rhclm.tex <==
\begin{algorithm}[htbp]
\caption{Random direction Hill-Climbing Linear Model(RHCLM)}
\begin{algorithmic}[1]
    \renewcommand{\algorithmicrequire}{\textbf{parameter(s):}}
    \renewcommand{\algorithmicensure}{\textbf{output:}}
    \REQUIRE $P$ - Population, $R$ - Fitness scores, $C$ - Number of Estimated individuals, $V$ - Number of steps
    \ENSURE  $L$ - Best estimated individuals
\\ \textit{Initialisation}
    \STATE $Q$←LINEAR-MODEL-Function with random weights $\theta$
    \STATE train $Q(P, R, \theta)$
    \COMMENT{Train surrogate model}
    \STATE $B \gets$ SORT-BY-ASC-SCORE($P$, $R$)
    \STATE $B \gets B[1:C]$
    % $Q$ - Surrogate model, $C$ - Number of genes, $V$ - Number of steps, $U$ - Best individuals
    \STATE $L  \gets RHC(Q_{\theta}, SIZE(B[1]), V, B)$
    \COMMENT{Algorithm 2}
    \RETURN $L$
\end{algorithmic} 
\end{algorithm}

==> datasets/results.tex <==
% \usepackage{filecontents}









==> equations/ampf.tex <==
The adaptive Mutation Probability Function follows as:

\[(\hat{\beta_0}, \hat{\beta_1}) = \arg\min_{b_0, b_1} \sum^n_{i=1}(Y_i - b_0 - b_1 \cdot X_i)^2\]

\begin{equation}
f(Y, X) = 1.5 - \frac{1}{1 + e^{-\alpha \cdot |\hat{\beta_1}|}} \label{ampf} 
\end{equation}

where $Y$ represents fitness scores of blackbox function and $X$ represents sequences of scores(0:1) and $\hat{\beta_0}$ represents intercept of linear regression of scores and $\hat{\beta_1}$ represents slope of linear regression of scores and $\alpha$ represents intensity factor of probability, when the value increases the probability increases stingy($1 \le \alpha, default=2$)



==> equations/reversed-func-id.tex <==
\[T=\{ \tau \in T^M | \tau \sim U_{(0,1)}\}\]
\[X' = \{X, T\}, Y'=\{Y, T\}\]
\[X'=\{x \in X'^{M \times (H+1)}\}, Y'=\{y \in Y'^{M \times 2}\}\] 
\begin{equation}
f^{-1}(Y') = X'
\end{equation}


==> equations/reversed-func.tex <==
\[X=\{x \in X^{M \times H}\}, Y=\{y \in Y^{N}\}, M \ge N\]
\[f(X)=Y\]
\begin{equation}
f^{-1}(Y)\not \neq X
\end{equation}

==> figures/ampf-eval-table.tex <==

\begin{table}[h!]
\caption{95 Confidence Interval Evaluation of Adaptive Mutation Probability Function(AMPF) vs. Epsilon Greedy0.5(EG0.5) }
\label{xgb-perf-table}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{|c|r|r|r|}
\hline
Algorithm& 
Test Loss& 
Valid Loss& 
Time(sec)\\
\hline

GA+AMPF&	0.17894±0.049293&	{\textbf{0.03291±0.013098}}&	133.35120±38.760646\\
GA+EG0.5&	0.16965±0.045888&	0.03923±0.016853&	120.33270±33.550151\\
\hline
\end{tabular}
% \label{tab1}
\end{table}


==> figures/chromosome-desc.tex <==
$
\text{a chromosome} = \underset{type: mlp}{00000000|} \underset{batch: 16}{00000010|} \underset{lr: 1e-2}{00000010|} \underset{type: uniform}{00000011|} \underset{depth: 4}{00000100|} \underset{neurons: 8}{00000011|} \underset{opt: adam}{00000011|} \underset{act: relu}{00000001|} \underset{init: he}{00000000}
$

==> figures/ci-nn-table.tex <==
\begin{table}
\caption{Performance of Neuralnet HPOBench}
\label{xgb-perf-table}
\setlength{\tabcolsep}{3pt}
% {|p{40pt}|p{60pt}|p{60pt}|p{60pt}|}
\begin{tabular}{|c|r|r|r|}
\hline
Algorithm& 
Test Loss& 
Valid Loss& 
Time(sec)\\
\hline
RGHL&	0.1774±0.008625&	{\textbf{0.0430±0.003274}}&	12303.170±1477.50701\\
RGHB&	0.1676±0.008550&	0.0449±0.003340&	17752.706±2206.44557\\
RS&	0.3067±0.017417&	0.2876±0.008102&	808.547±0038.85767\\
BO&	0.1537±0.007543&	0.0789±0.005616&	712.431±0025.77543\\
BOHB&	0.1667±0.006390&	0.0950±0.005909&	927.046±0015.13001\\
SMAC&	0.1677±0.008242&	0.0459±0.003699&	5577.922±0627.60109\\

\hline
\end{tabular}
% \label{tab1}
\end{table}

==> figures/ci-rf-table.tex <==
\begin{table}
\caption{Performance of RF HPOBench}
\label{xgb-perf-table}
\setlength{\tabcolsep}{3pt}
% {|p{40pt}|p{60pt}|p{60pt}|p{60pt}|}
\begin{tabular}{|c|r|r|r|}
\hline
Algorithm& 
Test Loss& 
Valid Loss& 
Time(sec)\\
\hline
RGHL&	0.1684±0.006773 &	0.0412±0.002238 &	123.597146±6.188801 \\
RGHB&	0.1667±0.006502 &	{\textbf{0.0407±0.002348 }}&	147.708267±5.552665 \\
RS&	0.2102±0.008689 &	0.5008±0.016402 &	121.677629±2.104253 \\
BO&	0.1712±0.006910 &	0.0527±0.002758 &	221.799096±5.050753 \\
BOHB&	0.1690±0.006763 &	0.0818±0.003877 &	672.364848±2.492630 \\
SMAC&	0.1708±0.006713 &	0.0411±0.002348 &	334.240021±6.427550 \\

\hline
\end{tabular}
% \label{tab1}
\end{table}

==> figures/ci-svm-table.tex <==
\begin{table}
\caption{Performance of SVM HPOBench}
\label{xgb-perf-table}
\setlength{\tabcolsep}{3pt}
% {|p{40pt}|p{60pt}|p{60pt}|p{60pt}|}
\begin{tabular}{|c|r|r|r|}
\hline
Algorithm& 
Test Loss& 
Valid Loss& 
Time(sec)\\
\hline
RGHL&	0.3009±0.013811 &	0.0548±0.003662 &	14.949991±1.226181 \\
RGHB&	0.3084±0.015773 &	0.0708±0.004270 &	74.199489±3.253045 \\
RS&	0.4534±0.014416 &	0.5351±0.013855 &	14.991651±0.953568 \\
BO&	0.2077±0.007916 &	0.0569±0.002816 &	62.234121±1.384060 \\
BOHB&	0.2378±0.010158 &	0.0933±0.003862 &	563.529929±1.172031 \\
SMAC&	0.1821±0.008033 &	{\textbf{0.0529±0.002517 }}&	118.696979±1.012420\\


\hline
\end{tabular}
% \label{tab1}
\end{table}

==> figures/ci-xgb-table.tex <==
\begin{table}
\caption{Performance of XGB HPOBench}
\label{xgb-perf-table}
\setlength{\tabcolsep}{3pt}
% {|p{40pt}|p{60pt}|p{60pt}|p{60pt}|}
\begin{tabular}{|c|r|r|r|}
\hline
Algorithm& 
Test Loss& 
Valid Loss& 
Time(sec)\\
\hline
RGHL&	0.1858±0.007484&	{\textbf{0.0372±0.002226}}&	419.962484±44.952676\\
RGHB&	0.1787±0.007153&	0.0441±0.002588&	442.980967±45.393322\\
RS&	0.1851±0.007007&	0.6696±0.009390&	206.583917±20.912707\\
BO&	0.1829±0.007253&	0.0530±0.002928&	326.795026±27.579218\\
BOHB&	0.1776±0.007311&	0.0708±0.003317&	793.597957±21.065918\\
SMAC&	0.1820±0.007156&	0.0390±0.002341&	416.835349±34.106769\\


\hline
\end{tabular}
% \label{tab1}
\end{table}

==> figures/dataset-spec-table.tex <==
\begin{table}
\caption{OpenML-CC18 Classification benchmark dataset}
\label{openml-dataset-spec-table}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{|c|l|r|r|r|}
\hline
Task-id& 
Name& 
\# of classes&
\# of features&
\# of instances\\
\hline
167151&	balance-scale&	3&	5&    625 \\
167154&	breast-w&	2&	10&    699 \\
167156&	mfeat-morphological&	10&	7& 2,000   \\
167163&	diabetes&	2&	9& 768 \\
167168&	vehicle&	4&	19& 846 \\
167187&	ilpd&	2&	11&    583 \\
167183&	banknote-authentication&	2&	5&  1,372   \\
167184&	blood-transfusion&	2&	5&   748 \\
167106&	climate-model&	2&	21&  540 \\
% 167184&	blood-transfusion-service-center&	2&	5& 748\\
% 167106&	climate-model-simulation-crashes&	2&	21& 540\\
\hline
% \multicolumn{5}{p{251pt}}{Vertical lines are optional in tables. Statements that serve as captions for 
% the entire table do not need footnote letters. }\\
% \multicolumn{5}{p{251pt}}{$^{\mathrm{a}}$Gaussian units are the same as cg emu for magnetostatics; Mx 
% $=$ maxwell, G $=$ gauss, Oe $=$ oersted; Wb $=$ weber, V $=$ volt, s $=$ 
% second, T $=$ tesla, m $=$ meter, A $=$ ampere, J $=$ joule, kg $=$ 
% kilogram, H $=$ henry.}
\end{tabular}
% \label{tab1}
\end{table}




==> figures/miso-vs-mimo-table.tex <==
% [6 rows x 112 columns]
%          Mean          CI
% 0    0.167359    0.020135
% 1    0.036647    0.006934
% 2  791.651570  220.684647
% 3    0.167677    0.020201
% 4    0.047253    0.007777
% 5  668.088558  196.020506

\begin{table}
\caption{95 Confidence Interval Evaluation of MISO vs. MIMO }
\label{xgb-perf-table}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{|c|r|r|r|}
\hline
Algorithm& 
Test Loss& 
Valid Loss& 
Time(sec)\\
\hline

MISO&	0.167359±0.0201&	{\textbf{0.036647±0.0069}}&	791.651570±220.6846\\
MIMO&	0.167677±0.0202&	0.047253±0.0077&	668.088558±196.0205\\
\hline
\end{tabular}
% \label{tab1}
\end{table}

==> figures/xgbhpo-perf-table.tex <==
\begin{table}
\caption{Performance of XGB HPOBench}
\label{xgb-perf-table}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{|p{40pt}|p{60pt}|p{60pt}|p{60pt}|}
\hline
Algorithm& 
Test Loss& 
Valid Loss& 
Time(sec)\\
\hline
RGHL&	0.1770±0.110067&	\textcolor{blue}{\textbf{0.03911±0.035922}}&	412.628±771.128168\\
RGHB&	0.1767±0.108612&	0.04145±0.040099&	414.095±674.319110\\
% RPS+CB&	0.1747±0.110248&	0.04581±0.043920&	383.052±692.697009\\
% RPS+PR&	0.1770±0.108455&	0.04482±0.039053&	347.375±611.844053\\
% GA&	0.1802±0.112457&	0.04883±0.043131&	288.734±502.738972\\
RS&	\textcolor{red}{\textbf{0.1829±0.106361}}&	\textcolor{red}{\textbf{0.06830±0.142725}}&	\textcolor{blue}{\textbf{204.796±327.512955}}\\
BO&	\textcolor{blue}{\textbf{0.1720±0.107543}}&	0.05118±0.044244&	304.338±367.382390\\
BOHB&	0.1771±0.108643&	0.06767±0.051013&	\textcolor{red}{\textbf{787.860±315.127910}}\\
SMAC&	0.1774±0.107909&	0.03921±0.035217&	398.177±482.016447\\

%RHC+CB&	0.176724±0.1086117014&	0.0414489±0.0400990522&	414.095±674.3191104697\\
%RPS+CB&	0.174659±0.1102475863&	0.0458098±0.0439199425&	383.052±692.6970087837\\
%RPS+PR&	0.177008±0.1084551062&	0.0448153±0.0390530352&	347.375±611.8440530023\\
%RPS+LR&	0.177038±0.1100667242&	0.0391127±0.0359215581&	412.628±771.1281680052\\
%GA&	0.180181±0.1124567180&	0.0488257±0.0431308431&	288.734±502.7389724424\\
%RS&	0.182904±0.1063605873&	0.0682959±0.1427249659&	204.796±327.512955490\\
%BO&	0.172076±0.1075431800&	0.0511816±0.0442438354&	304.338±367.382390103\\
%BOHB&	0.177059±0.1086429378&	0.0676650±0.0510129969&	787.860±315.12791042\\
%SMAC&	0.177398±0.1079089633&	0.0392055±0.0352166947&	398.177±482.01644745\\

\hline
\multicolumn{4}{p{251pt}}{Vertical lines are optional in tables. Statements that serve as captions for 
the entire table do not need footnote letters. }\\
\multicolumn{4}{p{251pt}}{$^{\mathrm{a}}$Gaussian units are the same as cg emu for magnetostatics; Mx 
$=$ maxwell, G $=$ gauss, Oe $=$ oersted; Wb $=$ weber, V $=$ volt, s $=$ 
second, T $=$ tesla, m $=$ meter, A $=$ ampere, J $=$ joule, kg $=$ 
kilogram, H $=$ henry.}
\end{tabular}
% \label{tab1}
\end{table}
